Attribute First, then Generate: Locally-attributable Grounded Text Generation

Recent efforts to address hallucinations in Large Language Models (LLMs) have focused on attributed text generation, which supplements generated texts with citations of supporting sources for post-generation fact-checking and corrections. Yet, these citations often point to entire documents or paragraphs, burdening users with extensive verification work. In this paper, we introduce a locally-attributable text generation approach, prioritizing concise attributions. Our method, named "Attribute First, then Generate", breaks down the conventional end-to-end generation process into three intuitive steps: content selection, sentence planning, and sequential sentence generation. By initially identifying relevant source segments ("select first") and then conditioning the generation process on them ("then generate"), we ensure these segments also act as the output's fine-grained attributions ("select" becomes "attribute"). Tested on Multi-document Summarization and Long-form Question-answering, our method not only yields more concise citations than the baselines but also maintains - and in some cases enhances - both generation quality and attribution accuracy. Furthermore, it significantly reduces the time required for fact verification by human assessors.

==> resources/MDS_regular_FiC_prompt.tex <==
\begin{figure*}[t]

\lstdefinestyle{promptStyle}
{
    basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
    numbers=left,numberstyle=\footnotesize,
    xleftmargin=2.8em,% show line numbers, remove this entire line if you don't want the numbers.
    xrightmargin=1.5em,
    showstringspaces=false,
      showspaces=false,
        showtabs=false,
    tabsize=2,
    breaklines=true,
        flexiblecolumns=true,
        escapeinside={<@}{@>},
          breakatwhitespace=true
}

\newtcblisting{mylisting}[1]{
  enhanced,
  listing only,
  boxrule=0.8pt,
  sharp corners=downhill,
  top=0mm,
  bottom=0mm,
  left=2mm,
  right=0mm,
  boxsep=0mm,
  colframe=black,
  colback=white,
  listing options={
    style=#1
  }
}

\definecolor{instructionsColor}{rgb}{0.1, 0.5, 0.1}

\begin{mylisting}{promptStyle}
<@\textcolor{instructionsColor}{In this task, you are presented with several passages, where some parts are "highlighted" (namely, there are <highlight\_start> and <highlight\_end> tokens before and after each such span). Your job is to generate a coherent summary that covers all and only the "highlighted" spans. Make sure ALL highlights are included. IMPORTANT: make sure that the summary consists of approximately 200 words and at least 7 sentences.}@>

<@\color{orange}Document [1]:@> <highlight_start>The United States on Wednesday warned US citizens<highlight_end> of a possible spike in "terrorist activity" in Colombia in the coming week as the left-wing Revolutionary Armed Forces of Colombia (FARC) <highlight_start>mark the one-year anniversary of the death of one of their commanders<highlight_end> ... 
<@\color{orange}Document [2]:@> <highlight_start>Colombia's hardline government said<highlight_end> Friday <highlight_start>it is willing to meet with members of the country's main leftist rebel group<highlight_end> in an unprecedented offer aimed at freeing dozens of rebel hostages, including three Americans ...
...

<@\color{blue}The highlighted spans are:@>
<@\color{orange}Document [1]:@> 
 1. The United States on Wednesday warned US citizens
 2. mark the one-year anniversary of the death of one of their commanders
...
<@\color{orange}Document [2]:@> 
 7. Colombia's hardline government said
 8. it is willing to meet with members of the country's main leftist rebel group 
...
<@\color{red}Answer:@> 
<@\color{blue}So the summary is:@> Colombia's strict government agreed to meet with the Country's main leftist rebel group. ...

<@\textcolor{instructionsColor}{In this task, you are presented with several passages, where some parts are "highlighted" (namely, there are <highlight\_start> and <highlight\_end> tokens before and after each such span). Your job is to generate a coherent summary that covers all and only the "highlighted" spans. Make sure ALL highlights are included. IMPORTANT: make sure that the summary consists of approximately 200 words and at least 7 sentences.}@>

<@\color{orange}Document [1]:@> <highlight_start>Voters in 11 states will pick their governors tonight<highlight_end>, and Republicans appear on track to increase their numbers by at least one, with the potential to extend their hold to more than two-thirds of the nation's top state offices ...
<@\color{orange}Document [2]:@> Eight of the gubernatorial seats up for grabs today are now held by Democrats; three are in Republican hands. <highlight_start>Republicans currently hold 29 governorships, Democrats have 20<highlight_end> ...
...

<@\color{blue}The highlighted spans are:@>
<@\color{orange}Document [1]:@> 
 1. Voters in 11 states will pick their governors tonight
...
<@\color{orange}Document [2]:@> 
 5. Republicans currently hold 29 governorships, Democrats have 20
...
<@\color{red}Answer:@> 
<@\color{blue}So the summary is:@>
\end{mylisting}
% \newtcbinputlisting[caption=Example prompt provided to GPT-4., frame=tlrb, captionpos=b]{figures/prompt.txt}
\caption{Example prompt for the fusion part of the plan recovery approach in the MDS setting.}
\label{fig:MDS_regular_FiC_prompt}
\end{figure*}

==> sections/6_analyses.tex <==
\section{Analyses}\label{sec:analyses}
To further investigate the quality of our pipeline both in terms of attribution and the overall tasks, we perform several analyses.

\paragraph{The Length-accuracy Tradeoff.}
In our human evaluation of attribution quality, annotators differentiated between fully unsupported and partially unsupported attributions. Despite treating the latter as non-attributed when calculating the AIS score, we aimed to further investigate them. 
Our analyses reveal that around 56\% of the 82 sentences deemed ``partially-attributed'' had unsupported information in immediate proximity to the cited spans, often within the same sentence for sub-sentence attributions.\footnote{see partially-attributed examples in \cref{sec:partially-attributing-examples}.} 
This observation suggests an inherent tradeoff between attribution brevity and fidelity.
Moreover, our analyses show that extending attributions from sub-sentence snippets to their corresponding full sentences improves the \textsc{AutoAIS} score, further pointing to this tradeoff (see \cref{sec:full_sentence_autoais}). 
These findings underscore the importance of further research into methods for improving adherence to cited content, particularly for fine-grained attributions.

% \paragraph{How can we boost the performance of fine-tuned models?}


% Our modular First-Attribute method allows for the integration of oracle gold annotations in place of original component outputs, providing a clearer insight into individual component errors and indicating the potential upper-bound performance achievable with current configurations. We explore replacing the content selection components with gold ``highlights'' and, where applicable, substituting the planning steps with oracle clusters. As detailed in \cref{appendix:oracle_results}, our experiments reveal that replacing predicted ``highlights'' with gold ones (``+ oracle highlights'' in \cref{tab:oracle_results_mds} and \cref{tab:oracle_results_lfqa}) significantly enhances the performance of both fine-tuned and ICL model variants on the original tasks. However, this substitution also tends to reduce the quality of attributions while also cutting the length of attributions by half.
% Moreover, incorporating oracle clusters for planning steps further boosts task performance and, in the case of fine-tuned models, improves attribution quality over using just oracle highlights. Conversely, this adjustment leads to an additional decline in attribution quality in the ICL variants.\looseness=-1

% The results indicate that despite the fine-tuned models' lower performance relative to ICL variants, they possess the potential to achieve comparable outcomes, particularly with optimized content selection.
% Yet, a more precise content selection possesses its own challenges, notably in adhering strictly to the selected, and often much shorter, content, potentially leading to unattributed outputs. These findings further accentuate the inherent tradeoff between attribution conciseness and compliance, observed in our analysis of partially-supporting attributions. This again emphasizes the need for further exploration into ways to ensure stricter compliance with the selected content, as well as to improve content selection precision, offering promising avenues for future research.


\begin{figure}[t]
\begin{adjustbox}{center}
    \centering
    \includegraphics[width=0.8\columnwidth]{resources/prefix_vs_no_prefix_thr.png}
\end{adjustbox}
    \caption{Percentage of more cohesive sentences when including the prefix in the input across varying upper limits of sentence index in the output.}
    \label{fig:prefix_vs_no_prefix_thr}
    
\end{figure}


\paragraph{Do models benefit from seeing the prefix?}
We also examine whether providing models with the context of previously generated sentences aids the generation process, particularly in enhancing output cohesion as defined by \citet{maimon2023novel}. Cohesion involves sentences being \textit{``referentially linked''}, e.g., via co-referring mentions, or linked through discourse connectors. 
To analyze the prefix's impact on cohesion, we modified the sentence generation prompt to exclude the prefix and conducted the sentence fusion step (step (c) in \cref{fig:architecture}) using the ICL variant for both MDS and LFQA tasks, maintaining identical sentence-level plans. 
Starting from the second sentence to isolate the prefix's impact, we examine 20 instances per task. Our analysis of 113 sentences reveals that approximately 30\% were more cohesive. Specifically, 23\% showed improved referential linkage, mostly attributed to better use of co-reference, and 7\% demonstrated better discourse connector usage.\footnote{See \cref{sec:prefix_vs_no_prefix} for examples.} 
Additionally, our findings suggest that prefixes play an increasing role in cohesion as the output progresses (see \cref{fig:prefix_vs_no_prefix_thr}), implying that cohesion gains importance as the text develops.\footnote{The observed plateau in cohesion levels in LFQA is attributed to its outputs generally not exceeding three sentences.}


==> sections/7_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Despite their impressive capabilities, LLMs have been shown to generate hallucinated content \cite{manakul2023selfcheckgpt, ji2023survey, huang2023survey}, emphasizing the need to verify their outputs. This has led to a growing interest in attributed generation, where models are encouraged to incorporate citations in their outputs. \citet{rashkin2022measuring} introduced the \textit{Attributed to Identified Sources} (AIS) framework for manually evaluating the reliability of generated statements through citations, while several works \cite[e.g.][]{bohnet2023attributed, gao-etal-2023-rarr} proposed using NLI models for automatic evaluation of citation alignment.

In Long-Form Question Answering (LFQA), the LaMDA system \citep{thoppilan2022lamda} was developed to support its answers with URLs, though these broad document citations lack conciseness for effective verification.  
On the other hand, GopherCite \citep{menick2022teaching} aimed to produce responses with fine-grained attribution, yet its approach lacks granularity in the \textit{output}, as it collectively attributes the entire generated text. In contrast, \citet{gao-etal-2023-enabling} proposed guiding LLMs to produce answers with inline citations to supporting \textit{documents} following each sentence (e.g., [1] to cite source 1), enhancing attribution granularity in the output but not in the input.
Moreover, strategies focusing on post-hoc attribution \citep{bohnet2023attributed, gao-etal-2023-rarr}, which involve retrieving and attributing potentially relevant passages after a model has generated a response, confront a significant combinatorial challenge, as they strive to accurately pair generated content with specific segments of source documents. Furthermore, they are often confined to paragraph- and sentence-level citations. 

\citet{schuster2023semqa}'s semi-extractive approach marks a notable advancement towards achieving both concise and comprehensive attributions. This method encourages models to copy verbatim spans from the source texts with minimal modifications for coherence, facilitating fine-grained attribution by design. However, its application is limited in scenarios requiring a higher level of abstraction, such as Multi-Document Summarization (MDS). 
In contrast to all those approaches, our proposed methodology is aimed to achieve fine-grained attribution both in the input and the output, without restricting the model to extractive text generation.

Another related line of research focuses on text-planning for improving output quality and reducing hallucinations~\citep{gehrmann-etal-2018-bottom, narayan-etal-2021-planning, narayan-etal-2023-conditional,zhao-etal-2020-bridging}, by introducing an additional step of planning before the final text generation. This area of study includes efforts to decompose the generation process into distinct phases, with some works focusing on the content-selection step \citep{gehrmann-etal-2018-bottom, cho-etal-2019-improving, ernst-etal-2021-summary}, while others focus on the content consolidation phase \citep{lebanoff-etal-2019-analyzing, lebanoff-etal-2020-learning, slobodkin-etal-2022-controlled, slobodkin-etal-2023-dont, hirsch-etal-2023-revisiting}. 
Our work also leverages this planning paradigm to improve the factuality of the output. However, unlike previous methods, our pipeline is carefully designed to also provide high-quality fine attributions.
Perhaps most related to our method is the work by \citet{ernst-etal-2022-proposition} that divides
% Notably, the work by \citet{ernst-etal-2022-proposition} closely mirrors our approach by dividing 
the MDS process into detecting salient propositions, clustering them, and transforming them into distinct sentences. However, their method results in outputs that resemble bullet-point summaries, consisting of single-proposition sentences, rather than producing the more fluid, multi-proposition sentences typical of natural text. In contrast, our method maintains the coherence and natural flow of generated texts without being restricted to single-proposition sentences.


==> sections/acknowledgements.tex <==
\section*{Acknowledgements}


==> tables/hyperparam_tuning_backtracking.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|ccc|ccc|}
\hline
        &     & \multicolumn{3}{c|}{MDS}                         & \multicolumn{3}{c|}{LFQA}                        \\
\# Demos & T   & R-L            & BERTScore      & AutoAIS        & R-L            & BERTScore      & AutoAIS        \\ \hline
1       & 0.1 & 21.10          & 87.06          & 53.31          & 40.57          & 91.22          & 61.52          \\
2       & 0.1 & 21.38          & 87.33          & 52.19          & 39.63          & 91.20          & 55.61          \\
3       & 0.1 & 20.86          & 86.97          & 51.97          & 43.14          & 91.83          & 68.64          \\
4       & 0.1 & -              & -              & -              & 42.20          & 91.63          & 64.66          \\
1       & 0.3 & 21.57          & 86.97          & 46.54          & 41.99          & 91.70          & 64.62          \\
2       & 0.3 & \textbf{22.44} & \textbf{87.27} & \textbf{54.11} & 41.68          & 91.77          & 64.96          \\
3       & 0.3 & 22.48          & 87.15          & 50.98          & \textbf{47.40} & \textbf{92.45} & \textbf{72.16} \\
4       & 0.3 & -              & -              & -              & 36.92          & 86.85          & 67.43          \\
1       & 0.5 & 21.33          & 86.70          & 46.22          & 44.46          & 91.85          & 58.33          \\
2       & 0.5 & 20.42          & 86.74          & 41.75          & 42.88          & 91.54          & 66.52          \\
3       & 0.5 & 22.07          & 86.59          & 53.56          & 40.38          & 91.25          & 64.90          \\
4       & 0.5 & -              & -              & -              & 43.45          & 91.47          & 66.70          \\
1       & 0.7 & 22.22          & 86.81          & 53.97          & 44.65          & 91.86          & 64.85          \\
2       & 0.7 & 20.45          & 86.63          & 44.79          & 42.14          & 91.54          & 65.49          \\
3       & 0.7 & 20.40          & 86.73          & 49.84          & 41.43          & 91.37          & 65.19          \\
4       & 0.7 & -              & -              & -              & 41.31          & 91.57          & 65.50          \\
1       & 0.9 & 21.06          & 86.91          & 47.95          & 41.38          & 91.28          & 70.64          \\
2       & 0.9 & 21.59          & 86.83          & 51.65          & 42.23          & 91.64          & 66.01          \\
3       & 0.9 & 21.91          & 86.89          & 57.72          & 43.21          & 89.92          & 61.43          \\
4       & 0.9 & -              & -              & -              & 41.46          & 91.38          & 62.16          \\ \hline
\end{tabular}%
}
\caption{Results on the development sets for the Few-shot variant when prompted to perform the final fusion of highlights using the backtracking strategy. We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric and for each setting (MDS or LFQA) are in bold.}
\label{tab:hyperparam_tuning_backtracking}
\end{table}

==> tables/oracle_full.tex <==


\begin{table*}[t!]
    \centering
    \small
    \adjustbox{max width=\textwidth}{
        \begin{tabular}{llcccc}
             & Method & \multicolumn{1}{c}{\textsc{Rouge$_L$$\uparrow$}} & \multicolumn{1}{c}{\textsc{BertScore$\uparrow$}} &  \multicolumn{1}{c}{\textsc{AutoAIS$\uparrow$}} & \multicolumn{1}{c}{\textsc{Length$\downarrow$}} \\
             \toprule
             \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ICL}}} & \textsc{Attr. First} & 16.7 & 85.2 & 80.6 & 92.7 \\
              & \hspace{3mm} {\smaller + oracle clusters} & 28.1 & 87.8 & 59.5 & 26.3 \\
              & \hspace{3mm} {\smaller + oracle highlights} & 20.2 & 86.6 & 61.3 & 44.3 \\
             % & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & 20.8 & 86.7 & 57.4 & 55.9 \\
              % & \hspace{3mm} {\smaller + oracle highlights} & 21.5 & 86.8 & 57.6 & 30.5 \\
             & \textsc{Attr. First\textsubscript{\texttt{CoT}}} & 19.5 & 86.1 &  71.2 & 75.3 \\
             & \hspace{3mm} {\smaller + oracle highlights} & 22.9 & 87.3 & 62.5 & 39.0 \\
             \midrule
             \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FT}}} & \textsc{Attr. First} & 16.5 & 84.9 & 64.4 & 33.1 \\
              & \hspace{3mm} {\smaller + oracle clusters} & 30.3 & 88.0 & 42.7 & 46.6 \\
              & \hspace{3mm} {\smaller + oracle highlights} & 21.6 & 86.8 & 32.9 & 21.6  \\
             % & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & 17.4 & 84.8 & 42.8 & 45.5 \\
              % & \hspace{3mm} {\smaller + oracle highlights} & 19.4 & 86.0 & 35.5 & 24.4 \\
             \bottomrule
        \end{tabular}
    }
    \caption{Results for the Multi-News MDS dataset oracle experiment conducted by replacing specific components with gold annotations.}
    \label{tab:oracle_results_mds}
\end{table*}

\begin{table*}[t!]
    \centering
    \small
    \adjustbox{max width=\textwidth}{
        \begin{tabular}{llcccc}
             & Method & \multicolumn{1}{c}{\textsc{Rouge$_L$$\uparrow$}} & \multicolumn{1}{c}{\textsc{BertScore$\uparrow$}} & \multicolumn{1}{c}{\textsc{AutoAIS$\uparrow$}} & \multicolumn{1}{c}{\textsc{Length$\downarrow$}} \\
             \toprule
             \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ICL}}} & \textsc{Attr. First} & 35.8 & 90.5 & 72.8 & 65.2 \\
             & \hspace{3mm} {\smaller + oracle clusters} & 45.5 & 92.2 & 64.8  & 24.8 \\
             & \hspace{3mm} {\smaller + oracle highlights} & 37.0 & 91.6  & 69.9 & 23.5 \\
             % & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & 38.9 & 91.8 & 72.0 & 49.4 \\
             % & \hspace{3mm} {\smaller + oracle highlights} & 36.3  & 91.1 & 58.2 & 20.1 \\
             & \textsc{Attr. First\textsubscript{\texttt{CoT}}} & 38.6 & 90.7 & 84.0 & 48.2 \\
             & \hspace{3mm} {\smaller + oracle highlights} & 47.7 & 92.7 & 81.5 & 29.5 \\
             \midrule
             \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{FT}}} & \textsc{Attr. First} & 24.7 & 88.0 & 52.7 & 20.9 \\
             & \hspace{3mm} {\smaller + oracle clusters} & 54.4 & 92.9 & 69.1 & 40.0 \\
             & \hspace{3mm} {\smaller + oracle highlights} & 44.3 & 86.8 & 51.1 & 27.7 \\
             % & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & 25.3 & 87.6 & 58.1 &  37.6 \\
             % & \hspace{3mm} {\smaller + oracle highlights} & 44.0 & 91.5 & 75.0 & 23.5 \\
             \bottomrule
             
        \end{tabular}
    }
    \caption{Results for LFQA dataset oracle experiment conducted by replacing specific components with gold annotations.}
    \label{tab:oracle_results_lfqa}
\end{table*}


==> tables/separate_hyperparam_tuning/hyperparam_tuning_LFQA_alce.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\# Demos & T   & R-L            & BERTScore      & AutoAIS        \\ \hline
1       & 0.1 & 37.25          & 90.12          & 71.13          \\
2       & 0.1 & 37.52          & 90.41          & 76.57          \\
3       & 0.1 & 37.24          & 90.19          & 72.46          \\
4       & 0.1 & 36.23          & 90.04          & 75.47          \\
1       & 0.3 & 36.78          & 90.17          & 75.08          \\
2       & 0.3 & 35.63          & 89.93          & 75.27          \\
3       & 0.3 & \textbf{39.05} & \textbf{90.51} & 72.24          \\
4       & 0.3 & 37.81          & 90.15          & 69.28          \\
1       & 0.5 & 35.02          & 89.75          & 71.36          \\
2       & 0.5 & 37.03          & 90.30          & \textbf{81.14} \\
3       & 0.5 & 36.68          & 90.01          & 73.64          \\
4       & 0.5 & 36.66          & 89.87          & 70.15          \\
1       & 0.7 & 36.02          & 89.68          & 64.91          \\
2       & 0.7 & 36.07          & 90.28          & 75.45          \\
3       & 0.7 & 33.33          & 89.80          & 72.17          \\
4       & 0.7 & 37.63          & 90.05          & 74.05          \\
1       & 0.9 & 35.33          & 90.01          & 75.46          \\
2       & 0.9 & 30.66          & 89.37          & 63.38          \\
3       & 0.9 & 33.64          & 89.52          & 72.58          \\
4       & 0.9 & 34.67          & 90.05          & 71.06          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the LFQA setting for the Few-shot variant when prompted to perform the ALCE variant. We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric are in bold.}
\label{tab:hyperparam_tuning_LFQA_alce}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_LFQA_clustering.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{|ccc|}
\hline
\# Demos & T   & F1             \\ \hline
1       & 0.1 & \textbf{70.91} \\
2       & 0.1 & 64.16          \\
3       & 0.1 & 68.01          \\
4       & 0.1 & 68.10          \\
1       & 0.3 & 54.34          \\
2       & 0.3 & 64.25          \\
3       & 0.3 & 54.46          \\
4       & 0.3 & 62.25          \\
1       & 0.5 & 59.56          \\
2       & 0.5 & 58.64          \\
3       & 0.5 & 58.14          \\
4       & 0.5 & 60.49          \\
1       & 0.7 & 56.74          \\
2       & 0.7 & 61.15          \\
3       & 0.7 & 63.13          \\
4       & 0.7 & 58.11          \\
1       & 0.9 & 53.12          \\
2       & 0.9 & 50.99          \\
3       & 0.9 & 56.04          \\
4       & 0.9 & 56.14          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the LFQA setting for the Few-shot variant when prompted for the clustering subtask. We tested different numbers of examples in the prompt and different temperatures. Best score is in bold.}
\label{tab:hyperparam_tuning_LFQA_clustering}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_LFQA_content_selection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{|ccc|}
\hline
\# Demos & T   & F1             \\ \hline
1       & 0.1 & 28.83          \\
2       & 0.1 & 29.22          \\
3       & 0.1 & 33.47          \\
4       & 0.1 & 34.10          \\
1       & 0.3 & 32.76          \\
2       & 0.3 & 31.78          \\
3       & 0.3 & 31.47          \\
4       & 0.3 & \textbf{34.81} \\
1       & 0.5 & 30.27          \\
2       & 0.5 & 28.61          \\
3       & 0.5 & 31.15          \\
4       & 0.5 & 29.20          \\
1       & 0.7 & 29.72          \\
2       & 0.7 & 28.88          \\
3       & 0.7 & 27.57          \\
4       & 0.7 & 32.45          \\
1       & 0.9 & 24.34          \\
2       & 0.9 & 30.12          \\
3       & 0.9 & 28.39          \\
4       & 0.9 & 33.12          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the LFQA setting for the Few-shot variant when prompted for the content selection subtask. We tested different numbers of examples in the prompt and different temperatures. Best score is in bold.}
\label{tab:hyperparam_tuning_LFQA_content_selection}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_FiC_CoT.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\# Demos & T   & R-L            & BERTScore      & AutoAIS        \\ \hline
1       & 0.1 & 23.52          & 87.63          & 56.88          \\
2       & 0.1 & 23.61          & 87.75          & 58.61          \\
3       & 0.1 & 24.91          & \textbf{88.07} & 58.24          \\
1       & 0.3 & 23.38          & 87.77          & 55.40          \\
2       & 0.3 & \textbf{25.32} & 88.05          & 57.65          \\
3       & 0.3 & 25.18          & 88.03          & 53.86          \\
1       & 0.5 & 23.28          & 87.85          & \textbf{59.58} \\
2       & 0.5 & 23.31          & 87.65          & 54.75          \\
3       & 0.5 & 24.24          & 87.93          & 51.16          \\
1       & 0.7 & 22.75          & 87.67          & 53.54          \\
2       & 0.7 & 24.00          & 87.90          & 54.53          \\
3       & 0.7 & 22.54          & 87.74          & 52.98          \\
1       & 0.9 & 22.54          & 87.49          & 56.15          \\
2       & 0.9 & 20.44          & 87.34          & 48.29          \\
3       & 0.9 & 22.75          & 87.47          & 42.54          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted to perform the final fusion of highlights using the Chain-of-Thought strategy. We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric are in bold.}
\label{tab:hyperparam_tuning_MDS_FiC_CoT}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_alce.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\# Demos & T   & R-L            & BERTScore      & AutoAIS        \\ \hline
1       & 0.1 & 19.90          & 86.45          & 92.34          \\
2       & 0.1 & 20.68          & 86.50          & 95.92          \\
3       & 0.1 & 21.09          & 86.47          & 95.64          \\
1       & 0.3 & 19.52          & 86.26          & 91.77          \\
2       & 0.3 & 20.87          & 86.48          & 94.79          \\
3       & 0.3 & 21.18          & 86.66          & 98.65          \\
1       & 0.5 & 19.75          & 86.50          & 93.82          \\
2       & 0.5 & \textbf{21.26} & 86.64          & \textbf{98.78} \\
3       & 0.5 & 20.78          & 86.42          & 95.85          \\
1       & 0.7 & 19.45          & 86.16          & 90.06          \\
2       & 0.7 & 20.95          & 86.48          & 95.75          \\
3       & 0.7 & 21.14          & \textbf{86.71} & 98.38          \\
1       & 0.9 & 19.58          & 86.21          & 91.42          \\
2       & 0.9 & 20.35          & 86.37          & 94.97          \\
3       & 0.9 & 20.18          & 86.33          & 94.13          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted to perform the ALCE variant. We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric are in bold.}
\label{tab:hyperparam_tuning_MDS_alce}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_backtracking.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\# Demos & T   & R-L            & BERTScore      & AutoAIS        \\ \hline
1       & 0.1 & 21.10          & 87.06          & 53.31          \\
2       & 0.1 & 21.38          & 87.33          & 52.19          \\
3       & 0.1 & 20.86          & 86.97          & 51.97          \\
1       & 0.3 & 21.57          & 86.97          & 46.54          \\
2       & 0.3 & \textbf{22.44} & \textbf{87.27} & \textbf{54.11} \\
3       & 0.3 & 22.48          & 87.15          & 50.98          \\
1       & 0.5 & 21.33          & 86.70          & 46.22          \\
2       & 0.5 & 20.42          & 86.74          & 41.75          \\
3       & 0.5 & 22.07          & 86.59          & 53.56          \\
1       & 0.7 & 22.22          & 86.81          & 53.97          \\
2       & 0.7 & 20.45          & 86.63          & 44.79          \\
3       & 0.7 & 20.40          & 86.73          & 49.84          \\
1       & 0.9 & 21.06          & 86.91          & 47.95          \\
2       & 0.9 & 21.59          & 86.83          & 51.65          \\
3       & 0.9 & 21.91          & 86.89          & 57.72          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted to perform the final fusion of highlights using the backtracking strategy . We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric are in bold.}
\label{tab:hyperparam_tuning_MDS_backtracking}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_clustering.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{|ccc|}
\hline
\# Demos & T   & F1             \\ \hline
1       & 0.1 & 27.58          \\
2       & 0.1 & 30.28          \\
3       & 0.1 & 31.96          \\
1       & 0.3 & 29.63          \\
2       & 0.3 & 31.87          \\
3       & 0.3 & 31.20          \\
1       & 0.5 & 29.57          \\
2       & 0.5 & \textbf{34.91} \\
3       & 0.5 & 33.31          \\
1       & 0.7 & 26.35          \\
2       & 0.7 & 29.89          \\
3       & 0.7 & 31.05          \\
1       & 0.9 & 26.60          \\
2       & 0.9 & 29.32          \\
3       & 0.9 & 29.34          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted for the clustering subtask. We tested different numbers of examples in the prompt and different temperatures. Best score is in bold.}
\label{tab:hyperparam_tuning_MDS_clustering}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_content_selection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{|ccc|}
\hline
\# Demos & T   & Tokens IoU     \\ \hline
1       & 0.1 & 29.81          \\
2       & 0.1 & \textbf{34.65} \\
3       & 0.1 & 33.29          \\
1       & 0.3 & 28.99          \\
2       & 0.3 & 32.29          \\
3       & 0.3 & 31.38          \\
1       & 0.5 & 29.56          \\
2       & 0.5 & 30.70          \\
3       & 0.5 & 30.76          \\
1       & 0.7 & 30.20          \\
2       & 0.7 & 26.28          \\
3       & 0.7 & 29.76          \\
1       & 0.9 & 25.29          \\
2       & 0.9 & 24.79          \\
3       & 0.9 & 30.15          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted for the content selection subtask. We tested different numbers of examples in the prompt and different temperatures. Best score is in bold.}
\label{tab:hyperparam_tuning_MDS_content_selection}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_e2e.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{|cccc|}
\hline
\# Demos & T   & R-L   & BERTScore \\ \hline
0       & 0.1 & 20.41 & 86.59     \\ 
1       & 0.1 & 20.76 & 86.60     \\ 
2       & 0.1 & 20.18 & 86.66     \\ 
3       & 0.1 & 20.53 & 86.77     \\ 
0       & 0.3 & 19.51 & 86.45     \\ 
1       & 0.3 & 20.36 & 86.63     \\ 
2       & 0.3 & 20.76 & 86.62     \\ 
3       & 0.3 & 20.44 & 86.55     \\ 
0       & 0.5 & 19.99 & 86.38     \\ 
1       & 0.5 & \textbf{21.04} & \textbf{86.83}     \\ 
2       & 0.5 & 20.23 & 86.49     \\ 
3       & 0.5 & 20.44 & 86.77     \\ 
0       & 0.7 & 20.70 & 86.38     \\ 
1       & 0.7 & 20.88 & 86.43     \\ 
2       & 0.7 & 20.00 & 86.67     \\ 
3       & 0.7 & 19.03 & 86.29     \\ 
0       & 0.9 & 18.89 & 85.93     \\ 
1       & 0.9 & 19.39 & 86.25     \\ 
2       & 0.9 & 20.06 & 86.38     \\ 
3       & 0.9 & 19.39 & 86.34     \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted to perform the full MDS task. We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric are in bold.}
\label{tab:hyperparam_tuning_MDS_e2e}
\end{table}

==> tables/separate_hyperparam_tuning/hyperparam_tuning_MDS_iterative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\# Demos & T   & R-L            & BERTScore      & AutoAIS        \\ \hline
1       & 0.1 & 26.92          & 87.34          & 45.81          \\
2       & 0.1 & 29.99          & 87.90          & 46.95          \\
3       & 0.1 & 29.83          & 87.97          & 51.22          \\
1       & 0.3 & 26.80          & 87.43          & 46.62          \\
2       & 0.3 & \textbf{30.53} & 87.94          & 47.61          \\
3       & 0.3 & 29.63          & 87.85          & \textbf{55.59} \\
1       & 0.5 & 28.78          & 87.76          & 46.45          \\
2       & 0.5 & 27.46          & 87.60          & 47.26          \\
3       & 0.5 & 28.83          & \textbf{87.98} & 42.49          \\
1       & 0.7 & 24.16          & 86.96          & 44.94          \\
2       & 0.7 & 26.91          & 87.61          & 52.01          \\
3       & 0.7 & 27.04          & 87.63          & 54.05          \\
1       & 0.9 & 22.33          & 86.69          & 39.23          \\
2       & 0.9 & 23.98          & 87.00          & 42.39          \\
3       & 0.9 & 25.54          & 87.44          & 47.81          \\ \hline
\end{tabular}%
}
\caption{Results on the development set in the MDS setting for the Few-shot variant when prompted to perform the final fusion of highlights using the iterative sentence-by-sentence strategy . We tested different numbers of examples in the prompt and different temperatures. Best scores on each metric are in bold.}
\label{tab:hyperparam_tuning_MDS_iterative}
\end{table}

==> tables/tab_ctr.tex <==
\begin{table*}
    \centering
    \small
    \adjustbox{max width=\textwidth}{
        \begin{tabular}{llcc|cccc}
            & Method & \multicolumn{1}{c}{\textsc{Rouge$_L$$\uparrow$}} & \multicolumn{1}{c}{\textsc{BertScore$\uparrow$}} & \multicolumn{1}{c}{\textsc{AutoAIS$\uparrow$}} & \multicolumn{1}{c}{\textsc{Length$\downarrow$}}& \multicolumn{1}{c}{\textsc{C. Val$\uparrow$}} & \multicolumn{1}{c}{\textsc{No Att. (\%)$\downarrow$}} \\
             \toprule
              \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ICL}}} & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & \textbf{20}.\textbf{8} & \textbf{86.7} & \textbf{57.4} & \textbf{55.9} & \textbf{1.03} & 0.0 \\
              &\hspace{3mm} {\smaller w/o re-generation} & 19.8 & 86.2 & 37.3 & 55.3 & 0.67 & 0.0 \\
             \midrule
             \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FT}}}  & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & 17.4 & 84.8 & \textbf{42.8} & \textbf{45}.\textbf{5} & \textbf{1}.\textbf{10} & 0.0 \\
                &\hspace{3mm} {\smaller w/o re-generation} & \textbf{18.2} & \textbf{85.5} & \textbf{42.8} & \textbf{45}.\textbf{5} & \textbf{1}.\textbf{10} & 0.0 \\

             \bottomrule
        \end{tabular}
    }
    % \vspace{-4pt}
    \caption{Recovery algorithm ablation results for MDS.}
    \label{tab:ctr_ablation_mds}
\end{table*}

\begin{table*}
    \centering
    \small
    \adjustbox{max width=\textwidth}{
        \begin{tabular}{llcc|cccc}
             & Method & \multicolumn{1}{c}{\textsc{Rouge$_L$$\uparrow$}} & \multicolumn{1}{c}{\textsc{BertScore$\uparrow$}} & \multicolumn{1}{c}{\textsc{AutoAIS$\uparrow$}} & \multicolumn{1}{c}{\textsc{Length$\downarrow$}}& \multicolumn{1}{c}{\textsc{C. Val$\uparrow$}} & \multicolumn{1}{c}{\textsc{No Att. (\%)$\downarrow$}} \\
             \toprule
             \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ICL}}} & \textsc{Attr. First\textsubscriptא{\texttt{recovery}}} & \textbf{38}.\textbf{9} & \textbf{91}.\textbf{8}  & \textbf{72.0} & \textbf{49.4} & \textbf{1.45} & 0.0 \\
             &\hspace{3mm} {\smaller w/o re-generation} & 37.4 & 90.5 & 41.8 & 49.4 & 0.84 & 0.0 \\
             \midrule
            \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{FT}}} & \textsc{Attr. First\textsubscript{\texttt{recovery}}} & \textbf{25.3} & \textbf{87.6} & \textbf{58.1} & \textbf{37}.\textbf{6} & \textbf{1.54} & 0.0 \\
            &\hspace{3mm} {\smaller w/o re-generation} & 23.7 & 87.1 & 47.4 & 41.0 & 1.15 & 0.0 \\
             \bottomrule
        \end{tabular}
    }
    % \vspace{-4pt}
    % \caption{Results for the long-form QA dataset derived from \citet{liu-etal-2023-evaluating} annotations.}
    \caption{Recovery algorithm ablation results for LFQA.}
    \label{tab:ctr_ablation_lfqa}
\end{table*}

==> tables/tab_prefix_experiment.tex <==

\begin{table}
    \centering
    \small
    \adjustbox{max width=\columnwidth}{
        \begin{tabular}{lccc}
             Method & \multicolumn{1}{c}{Fluency$\uparrow$} & \multicolumn{1}{c}{AIS$\uparrow$} & \multicolumn{1}{c}{Avg. time (sec)$\downarrow$} \\
             \toprule
             \textsc{ALCE} & 4.7 & \textbf{89.3} & 47 \\
             \textsc{Attr. First}\textsubscript{\texttt{ICL-CoT}} & \textbf{4.9} & 79.9 & \textbf{22} \\
             \bottomrule
        \end{tabular}
    }
    \caption{Results for the prefix experiment.}
    \label{tab:human_results_mds}
\end{table}

